Benchmarking Robustness of Multimodal Image-Text Models under Distribution Shift

Multimodal image-text models have shown remarkable performance in the past few years. However, evaluating robustness against distribution shifts is crucial before adopting them in real-world applications. In this work, we investigate the robustness of 12 popular open-sourced image-text models under common perturbations on five tasks (image-text retrieval, visual reasoning, visual entailment, image captioning, and text-to-image generation). In particular, we propose several new multimodal robustness benchmarks by applying 17 image perturbation and 16 text perturbation techniques on top of existing datasets. We observe that multimodal models are not robust to image and text perturbations, especially to image perturbations. Among the tested perturbation methods, character-level perturbations constitute the most severe distribution shift for text, and zoom blur is the most severe shift for image data. We also introduce two new robustness metrics (\textbf{MMI} for MultiModal Impact score and \textbf{MOR} for Missing Object Rate) for proper evaluations of multimodal models. We hope our extensive study sheds light on new directions for the development of robust multimodal models. More details can be found on the project webpage: \url{https://MMRobustness.github.io}.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/main/image_cap_blip.tex <==
\begin{tabular}{llrrrrrrrr}\toprule
& &\textbf{Bleu\_1} &\textbf{Bleu\_2} &\textbf{Bleu\_3} &\textbf{Bleu\_4} &\textbf{Meteor} &\textbf{Rouge\_L} &\textbf{CIDEr} \\
\midrule
\multirow{4}{*}{\textbf{Noise}} &\textbf{Gaussian} &70.9 &54.4 &41.3 &31.4 &26.1 &53.3 &100.5 \\
&\textbf{Shot} &71.9 &55.7 &42.6 &32.5 &26.8 &54.3 &104.3 \\
&\textbf{Impluse} &71.1 &54.8 &41.7 &31.7 &26.4 &53.7 &101.6 \\
&\textbf{Speckle} &74.8 &59.0 &45.8 &35.5 &28.5 &56.7 &116.5 \\
\midrule
\multirow{4}{*}{\textbf{Blur}} &\textbf{Defocus} &68.5 &52.3 &39.1 &29.1 &24.7 &50.9 &91.8 \\
&\textbf{Glass} &77.5 &62.3 &49.1 &38.4 &30.1 &58.8 &128.1 \\
&\textbf{Motion} &66.5 &50.0 &36.7 &26.8 &23.6 &49.3 &84.2 \\
&\textbf{Zoom} &55.9 &37.5 &24.4 &16.1 &17.0 &40.5 &45.9 \\
\midrule
\multirow{4}{*}{\textbf{Weather}} &\textbf{Snow} &70.6 &53.8 &40.5 &30.7 &25.7 &52.4 &95.7 \\
&\textbf{Frost} &73.4 &57.5 &44.3 &34.0 &27.7 &55.6 &111.6 \\
&\textbf{Fog} &75.0 &59.3 &45.9 &35.4 &28.8 &57.0 &116.1 \\
&\textbf{Brightness} &77.3 &61.8 &48.4 &37.8 &29.8 &58.6 &125.8 \\
\midrule
\multirow{4}{*}{\textbf{Digital}} &\textbf{Contrast} &71.3 &54.9 &41.6 &31.4 &25.7 &53.2 &98.3 \\
&\textbf{Elastic} &69.9 &53.4 &40.6 &30.9 &25.7 &52.7 &96.8 \\
&\textbf{Pixelate} &62.7 &45.4 &32.6 &23.8 &21.3 &46.8 &68.6 \\
&\textbf{JPEG} &76.2 &60.6 &47.4 &37.0 &29.3 &57.8 &121.8 \\
\midrule
\textbf{Stylize} &\textbf{Stylize} &63.7 &46.2 &32.9 &23.6 &21.1 &46.8 &68.7 \\
\midrule
\textbf{GT} &\textbf{GT} &78.9 &63.8 &50.5 &39.7 &31.0 &60.0 &133.3 \\
\bottomrule
\end{tabular}

==> tables/main/image_cap_grit.tex <==
\begin{tabular}{llrrrrrrrr}\toprule
& &\textbf{Bleu\_1} &\textbf{Bleu\_2} &\textbf{Bleu\_3} &\textbf{Bleu\_4} &\textbf{Meteor} &\textbf{Rouge\_L} &\textbf{CIDEr} \\
\midrule
\multirow{4}{*}{\textbf{Noise}} &\textbf{Gaussian} &78.6 &62.2 &47.6 &35.8 &27.0 &55.8 &117.4 \\
&\textbf{Shot} &79.1 &62.6 &48.1 &36.3 &27.2 &56.2 &118.6 \\
&\textbf{Impluse} &78.8 &62.4 &47.9 &36.1 &27.1 &56.0 &118.0 \\
&\textbf{Speckle} &81.1 &65.0 &50.5 &38.5 &28.4 &57.8 &128.1 \\
\midrule
\multirow{4}{*}{\textbf{Blur}} &\textbf{Defocus} &79.4 &63.1 &48.7 &36.9 &27.5 &56.6 &120.2 \\
&\textbf{Glass} &83.6 &68.4 &53.9 &41.5 &30.1 &60.1 &140.0 \\
&\textbf{Motion} &77.9 &61.3 &46.8 &35.2 &26.7 &55.4 &115.1 \\
&\textbf{Zoom} &60.0 &40.5 &27.1 &18.5 &17.7 &42.6 &56.1 \\
\midrule
\multirow{4}{*}{\textbf{Weather}} &\textbf{Snow} &78.6 &61.8 &47.2 &35.4 &27.0 &55.6 &118.1 \\
&\textbf{Frost} &81.8 &65.9 &51.4 &39.2 &28.8 &58.3 &131.1 \\
&\textbf{Fog} &83.1 &67.5 &53.0 &40.7 &29.6 &59.4 &136.6 \\
&\textbf{Brightness} &83.1 &67.7 &53.2 &40.9 &29.9 &59.8 &138.3 \\
\midrule
\multirow{4}{*}{\textbf{Digital}} &\textbf{Contrast} &81.4 &65.3 &50.7 &38.5 &28.5 &58.0 &128.4 \\
&\textbf{Elastic} &77.4 &60.5 &46.1 &34.6 &26.2 &55.0 &110.6 \\
&\textbf{Pixelate} &64.0 &44.3 &30.3 &20.9 &18.7 &44.5 &60.0 \\
&\textbf{JPEG} &81.6 &65.8 &51.2 &39.1 &28.9 &58.4 &131.1 \\
\midrule
\textbf{Stylize} &\textbf{Stylize} &68.9 &50.0 &35.5 &25.3 &21.2 &48.2 &77.4 \\
\midrule
\textbf{GT} &\textbf{GT} &84.2 &69.1 &54.7 &42.3 &30.6 &60.7 &144.0 \\
\bottomrule
\end{tabular}

==> tables/main/quality.tex <==
\begin{tabular}{l |  c | c c c c | c c c c | c c c c | c c c c |c }
\toprule
SSIM / LPIPS & \multicolumn{1}{c|}{\,Clean\,} & \tiny{Gauss.}
    & \tiny{Shot} & \tiny{Impulse} & \tiny{Speckle} & \tiny{Defocus} & \tiny{Glass} & \tiny{Motion} & \tiny{Zoom}~ & ~\tiny{Snow} & ~\tiny{Frost}~ & ~\tiny{Fog} & ~\tiny{Bright} & \tiny{Contrast} & \tiny{Elastic} & \tiny{Pixel} & \tiny{JPEG}~ &\tiny{Stylize}  
    \\
\midrule
1 &1.00/0.00&0.61/0.26  &0.65/0.25  &0.58/0.37  &0.72/0.20  &0.65/0.30  &0.78/0.25  &0.70/0.24  &0.68/0.20  &0.66/0.24  &0.68/0.20  &0.63/0.17  &0.79/0.12  &0.67/0.17  &0.66/0.26  &0.72/0.22  &0.78/0.17  &0.72/0.21   \\
2 &1.00/0.00&0.49/0.42  &0.52/0.42  &0.45/0.55  &0.66/0.28  &0.59/0.49  &0.73/0.34  &0.59/0.33  &0.57/0.36  &0.48/0.37  &0.58/0.28  &0.57/0.32  &0.70/0.21  &0.58/0.25  &0.53/0.29  &0.57/0.35  &0.67/0.23  &0.58/0.34 \\
3 &1.00/0.00&0.37/0.63  &0.41/0.60  &0.37/0.68  &0.51/0.51  &0.50/0.61  &0.58/0.47  &0.51/0.41  &0.50/0.44  &0.52/0.45  &0.53/0.34  &0.53/0.37  &0.65/0.31  &0.49/0.38  &0.42/0.39  &0.53/0.43  &0.65/0.35  &0.47/0.43  \\
4 &1.00/0.00&0.27/0.86  &0.29/0.85  &0.27/0.89  &0.34/0.63  &0.35/0.68  &0.48/0.60  &0.46/0.58  &0.47/0.58  &0.46/0.51  &0.53/0.44  &0.52/0.52  &0.53/0.48  &0.39/0.58  &0.41/0.52  &0.47/0.52 & 0.60/0.46  &0.37/0.52 \\
5 &1.00/0.00&0.19/0.99  &0.23/0.99  &0.19/0.99  &0.27/0.76  &0.32/0.72  &0.32/0.70  &0.33/0.61  &0.36/0.69  &0.32/0.63  &0.40/0.52  &0.38/0.64  &0.45/0.64  &0.33/0.73  &0.39/0.78  &0.37/0.63  &0.45/0.68  &0.31/0.67 \\
\bottomrule
\end{tabular}

==> tables/main/stable-diffusion-ttest.tex <==
\begin{tabular}{llrrrrrrr}\toprule
& &\multicolumn{2}{c}{\textbf{4 image}} &\multicolumn{2}{c}{\textbf{8 images}} &\multicolumn{2}{c}{\textbf{16 images}} \\
& &statistic &pvalue &statistic &pvalue &statistic &pvalue \\
\midrule
\multirow{6}{*}{Character-level} 
&\textbf{Keyboard} &-42.16 &0 &-50.67 &0 &-61.07 &0 \\
&\textbf{OCR} &-24.98 &0 &-31.2 &0 &-40.24 &0 \\
&\textbf{CI} &-35.61 &0 &-43.64 &0 &-53.76 &0 \\
&\textbf{CR} &-37.61 &0 &-44.39 &0 &-60.07 &0 \\
&\textbf{CS} &-39.67 &0 &-47.67 &0 &-57.62 &0 \\
&\textbf{CD} &-39.94 &0 &-48.18 &0 &-58.45 &0 \\
\midrule
\multirow{5}{*}{Word-level} 
&\textbf{SR} &-22.21 &0 &-28.3 &0 &-37.64 &0 \\
&\textbf{RI} &-11.64 &0 &-15.91 &0 &-24.12 &0 \\
&\textbf{RS} &-14.3 &0 &-19.36 &0 &-28.35 &0 \\
&\textbf{RD} &-9.37 &0 &-13.18 &0 &-21.31 &0 \\
&\textbf{IP} &-7.26 &0 &-10.33 &0 &-17.74 &0 \\
\midrule
\multirow{5}{*}{Sentence-level} 
&\textbf{Formal} &-2.96 &0 &-5.27 &0 &-12.22 &0 \\
&\textbf{Casual} &-3.58 &0 &-5.73 &0 &-12.37 &0 \\
&\textbf{Passive} &-5.15 &0 &-8.23 &0 &-15.33 &0 \\
&\textbf{Active} &-2.25 &0.02 &-3.88 &0 &-10.07 &0 \\
&\textbf{Back\_trans} &-7.09 &0 &-10.35 &0 &-17.58 &0 \\
\midrule
GT &\textbf{GT} &0 &1 &0 &1 &0 &1 \\
\bottomrule
\end{tabular}

==> tables/main/tasks_1.tex <==
\begin{tabular}{llllr}\toprule
Task & Datasets &Models & Evaluation metrics \\
\midrule
Image-text Retrieval &Flicker30K \cite{Young2014FromID}, COCO \cite{Lin2014MicrosoftCC} &CLIP \cite{Radford2021LearningTV}, TCL \cite{Yang2022VisionLanguagePW}, ALBEF \cite{Li2021AlignBF}, BLIP \cite{Li2022BLIPBL} & Recall K (R@K), K = $\{1, 5, 10\}$, and RSUM \cite{Karpathy2017DeepVA} \\
Visual Reasoning &NLVR2 \cite{Suhr2017ACO} & ALBEF \cite{Li2021AlignBF}, ViLT \cite{Kim2021ViLTVT}, BLIP \cite{Li2022BLIPBL}, TCL \cite{Yang2022VisionLanguagePW}, METER \cite{Dou2021AnES} & Prediction accuracy\\
Visual Entailment &SNLI-VE \cite{xie2018visual,xie2019visual} & ALBEF \cite{Li2021AlignBF}, TCL \cite{Yang2022VisionLanguagePW}, METER \cite{Dou2021AnES} & Prediction accuracy\\
Image Captioning &COCO \cite{Lin2014MicrosoftCC} &BLIP \cite{Li2022BLIPBL}, GRIT \cite{Nguyen2022GRITFA} &BLEU \cite{Papineni2002BleuAM}, METEOR \cite{Denkowski2014MeteorUL}, ROUGE-L \cite{Lin2004ROUGEAP}, CIDEr \cite{Vedantam2015CIDErCI} \\
Text-to-image Generation &COCO \cite{Lin2014MicrosoftCC} &Stable Diffusion \cite{Rombach2022HighResolutionIS}, GLIDE \cite{Nichol2022GLIDETP} & FID \cite{Heusel2017GANsTB}, CLIP-FID \cite{Kynkaanniemi2022TheRO,parmar2021cleanfid}\\
\bottomrule
\end{tabular}

==> tables/main/tasks_2.tex <==
\begin{tabular}{llllr}\toprule
Task & Datasets &Models & Evaluation metrics \\
\midrule
Image-text Retrieval &Flicker30K , COCO  &CLIP, TCL, ALBEF, BLIP & Recall K (R@K), K = $\{1, 5, 10\}$, and RSUM  \\
Visual Reasoning &NLVR2  & ALBEF, ViLT, BLIP, TCL, METER  & Prediction accuracy\\
Visual Entailment &SNLI-VE  & ALBEF, TCL, METER & Prediction accuracy\\
Image Captioning &COCO  &BLIP, GRIT  &BLEU, METEOR, ROUGE-L, CIDEr \\
Text-to-image Generation &COCO  &Stable Diffusion, GLIDE  & FID, CLIP-FID \\
\bottomrule
\end{tabular}

==> tables/main/text_example_old.tex <==
\begin{tabular}{ll|p{18cm}}
    \toprule
      Category & Perturbation  & Example   \\ 
    \midrule
    \multirow{1}{*}{Original } 
     &Clean  &A baseball player in red leaps into the air to avoid a player in blue who is shortly behind him as he catches the ball while other blue team members look on in the background.	 \\
     \midrule
     \multirow{9}{*}{Character} 
     &Keyboard  &A b\textcolor{orange}{z}ssball play\textcolor{orange}{d}r in red leap\textcolor{orange}{d} int\textcolor{orange}{P} the air to \textcolor{orange}{q}void a player in blue who is shortly be\textcolor{orange}{j}ind him as he catches the ball whil\textcolor{orange}{@} \textcolor{orange}{L}ther bl\textcolor{orange}{j}e team members \textcolor{orange}{K}ook on in the background. \\
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &OCR  &A baseball player in red leaps int\textcolor{orange}{0} the air to avoid a p\textcolor{orange}{1}ayer in b1ue wh\textcolor{orange}{0} i\textcolor{orange}{8} shortly behind him as he catches the ball whi\textcolor{orange}{1}e other b\textcolor{orange}{1}ue team members look on in the background.	 \\ 
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &CI  &	A baseb\textcolor{orange}{6}a1l player in red leaps into the air to avo\textcolor{orange}{0}id a player\textcolor{orange}{k} in blue who is s\textcolor{orange}{8}hort1y \textcolor{orange}b{6}ehind him as he catches\textcolor{orange}{8} the ball while other blue team members look\textcolor{orange}{r} \textcolor{orange}o{0}n in the background. \\
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &CR  &A baseball player in red \textcolor{orange}{1}eaps into the air to av\textcolor{orange}{b}id a player in blue who i\textcolor{orange}{8} shortly behind him as he catches the ball whi\textcolor{orange}{g}e other blue team members look on in the background.	 \\
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &CS &A baseball play\textcolor{orange}{re} in r\textcolor{orange}{de} leaps into the a\textcolor{orange}{ir} \textcolor{orange}{ot} avoid a player in blue who is shortly behind him \textcolor{orange}{sa} he catches the b\textcolor{orange}{la}l whi1e oth\textcolor{orange}{re} blue team m\textcolor{orange}{me}bers look on in the background.	 \\ 
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &CD &A baseball play\textcolor{orange}{\_}r in red leaps into the ai\textcolor{orange}{\_} to avoid a pl\textcolor{orange}{\_}yer in blue who is shortly behind him as he catc\textcolor{orange}{\_}es the ball wh\textcolor{orange}{\_}le other blue te\textcolor{orange}{\_}m members lo\textcolor{orange}{\_}k on in the back\textcolor{orange}{\_}round.	 \\
     \midrule
     \multirow{10}{*}{Word}
     &SR &A baseball \textcolor{orange}{histrion} in \textcolor{orange}{reddish} leaps into the \textcolor{orange}{bare} to \textcolor{orange}{fend off} a \textcolor{orange}{histrion }in \textcolor{orange}{dingy} who is in \textcolor{orange}{brief} behind him as he catches the ball while other \textcolor{orange}{dingy} team up members \textcolor{orange}{facial expression} on in the background.
	 \\  
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &WI  &A baseball player in \textcolor{orange}{inward role player} red leaps \textcolor{orange}{live} into \textcolor{orange}{exist} the air to avoid a player \textcolor{orange}{depressed} in blue who is shortly behind him as he catches the ball while other blue team members look on \textcolor{orange}{member angstrom} in \textcolor{orange}{captivate} the background.
	 \\ 
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &WS  &A \textcolor{orange}{in player} in red leaps \textcolor{orange}{ball the while} \textcolor{orange}{to} player \textcolor{orange}{a} avoid \textcolor{orange}{in blue} who is shortly \textcolor{orange}{on} him \textcolor{orange}{air blue} catches the \textcolor{orange}{into} as other \textcolor{orange}{he} team members look \textcolor{orange}{baseball behind} the background.
	 \\ 
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &WD  &A baseball \textcolor{orange}{[X]} in red leaps \textcolor{orange}{[X]} the air to avoid a player in blue who is shortly behind him as he catches the ball while other \textcolor{orange}{[X]} team members look on in the \textcolor{orange}{[X]}.
	 \\ 
     \cmidrule(l){2-2} \cmidrule(l){3-3}
     &IP &A baseball player in \textcolor{orange}{.} red \textcolor{orange}{:} leaps \textcolor{orange}{.} into \textcolor{orange}{?} the \textcolor{orange}{!} air \textcolor{orange}{!} to \textcolor{orange}{;} avoid a \textcolor{orange}{,} player in blue \textcolor{orange}{,} who \textcolor{orange}{?} is \textcolor{orange}{;} shortly \textcolor{orange}{.} behind \textcolor{orange}{,} him as \textcolor{orange}{.} he catches the \textcolor{orange}{,} ball while \textcolor{orange}{?} other blue team members look \textcolor{orange}{?} on in \textcolor{orange}{;} the background.	 \\ 
     \midrule
     \multirow{8}{*}{Sentence} 
     &Formal  &\textcolor{orange}{As} a baseball player in red leaps into the air to avoid a player in blue who is shortly behind him as he catches the ball.		  \\
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &Casual  &\textcolor{orange}{And as} a red baseball team player leaps in the air to avoid a blue team player that's \textcolor{orange}{close by} he catches the ball.		  \\
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &Passive  &The ball is \textcolor{orange}{spotted} by a baseball player in red as he is \textcolor{orange}{approached} by other blue team members.	  \\
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &Active  &A baseball player in red leaps into the air to avoid a player \textcolor{orange}{dressed} in blue  who is \textcolor{orange}{currently} shortly behind him as he catches the ball.	  \\
     \cmidrule(l){2-2} \cmidrule(l){3-3} 
     &Back\_trans  &A baseball player in red leaps into the air to \textcolor{orange}{dodge} a player in blue who is \textcolor{orange}{just} behind him as he catches the ball, while other blue team members \textcolor{orange}{watch }in the background.	  \\
    \bottomrule
\end{tabular}

==> tables/main/vr_ve_ip.tex <==
\begin{tabular}{l c |  c | c c c c | c c c c | c c c c | c c c c |c| c| c }
\toprule
\multicolumn{1}{c}{}
&\multicolumn{2}{c}{} & \multicolumn{4}{c}{Noise} & \multicolumn{4}{c}{Blur} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Digital} & \multicolumn{1}{c}{Stylize}& \multicolumn{1}{c}{}
& \multicolumn{1}{c}{}
\\ 
\midrule
Dataset &Method & \multicolumn{1}{c|}{\,Clean\,} & \tiny{Gauss.}
    & \tiny{Shot} & \tiny{Impulse} & \tiny{Speckle} & \tiny{Defocus} & \tiny{Glass} & \tiny{Motion} & \tiny{Zoom}~ & ~\tiny{Snow} & ~\tiny{Frost}~ & ~\tiny{Fog} & ~\tiny{Bright} & \tiny{Contrast} & \tiny{Elastic} & \tiny{Pixel} & \tiny{JPEG}~ &\tiny{Stylize}  & {\,\textbf{ave }\,} &\tiny{MMI} 
    \\
\midrule
\multirow{5}{*}{NLVR2-test} 
&ALBEF &83.14 &53.17 &52.85 &53.22 &53.50 &52.68 &53.09 &52.39 &\textbf{51.19} &51.60 &52.98 &\underline{53.49} &52.78 &53.13 &53.12 &51.72 &53.10 &52.95 &52.76  &\textcolor{blue}{$\downarrow$ 36.5\%} \\
&ViLT  &76.13 &74.24 &73.80 &74.43 &74.20 &72.32 &\underline{76.70} &72.55 &\textbf{62.34} &69.24 &73.36 &75.05 &74.73 &68.68 &74.07 &69.06 &76.52 &71.50 &72.54 &\textcolor{blue}{$\downarrow$ 4.7\%} \\
&TCL  &81.33 &78.10 &77.87 &78.25 &78.91 &78.00 &\underline{81.59} &78.17 &\textbf{67.81} &75.74 &79.62 &80.64 &81.52 &74.35 &79.76 &74.61 &81.28 &75.85 &77.77  &\textcolor{blue}{$\downarrow$ 4.4\%} \\
&BLIP  &83.08 &75.39 &75.39 &85.10 &72.31 &\underline{85.64} &79.49 &76.92 & \textbf{58.97} & 80.51 &75.90 &81.54 &76.92 &81.03 &77.95 &73.333 &78.97 &73.85 &77.01 &\textcolor{blue}{$\downarrow$ 7.3\%} \\
&METER &83.05 &78.87 &77.94 &77.78 &79.23 &78.97 &\underline{82.10} &79.14 &\textbf{68.89} &76.69 &80.10 &82.25 &81.21 &78.20 &79.91 &72.65 &80.74 &76.93 &78.34 &\textcolor{blue}{$\downarrow$ 5.7\%} \\
\midrule
\multirow{3}{*}{SNLI-VE-test} 
&ALBEF &80.91 &77.65 &77.70 &77.40 &78.50 &76.62 &79.25 &76.59 &\textbf{71.70} &76.31 &78.60 &78.47 &\underline{79.77} &78.07 &78.34 &74.42 &78.81 &74.89 &77.24 &\textcolor{blue}{$\downarrow$ 8.3\%} \\
&TCL &80.29 &77.46 &77.38 &77.30 &78.17 &76.80 &79.27 &75.56 &\textbf{71.07} &76.13 &78.24 &78.38 &\underline{79.19} &78.68 &77.74 &71.76 &78.59 &74.70 &76.85 &\textcolor{blue}{$\downarrow$ 4.3\%} \\
&METER &81.19 &77.16 &77.09 &76.90 &78.58 &77.14 &80.13 &77.39 &\textbf{74.35} &77.79 &79.84 &80.18 &\underline{80.46} &79.18 &78.91 &72.67 &79.32 &76.08 &77.79 &\textcolor{blue}{$\downarrow$ 4.2\%} \\
\bottomrule
\end{tabular}

==> tables/main/vr_ve_tp.tex <==
\begin{tabular}{l l|  c | c c c c c c| c c c c c | c c c c c | c |c} 
\toprule
\multicolumn{1}{c}{}
&\multicolumn{2}{c}{} & \multicolumn{6}{c}{Character-level} & \multicolumn{5}{c}{Word-level} & \multicolumn{5}{c}{Sentence-level} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}
\\ 
\midrule
Dataset &Method & \multicolumn{1}{c|}{\,Clean\,} & \tiny{Keyboard}
    & \tiny{OCR} & ~~~\tiny{CI}~~ & ~~~\tiny{CR}~~ & ~~~\tiny{CS}~~ & ~~~\tiny{CD}~~ & ~~~\tiny{SR}~~ & ~~~\tiny{WI}~~ & ~~~\tiny{WS}~~ & ~~~\tiny{WD}~~ & ~~~\tiny{IP}~~ & \tiny{Formal} & \tiny{Casual} & \tiny{Passive} & \tiny{Active} & \tiny{Back\_trans}  & {\,\textbf{ave }\,}
    & MMI \\ 
\midrule
\multirow{5}{*}{NLVR2-test} 
&ALBEF &83.14 &51.39 &51.99 &\textbf{51.04} &51.26 &51.05 &51.24 &52.69 &52.95 &52.95 &52.88 &53.30 &\underline{53.39} &53.06 &52.68 &53.26 &53.23 &52.40 &\textcolor{blue}{$\downarrow$ 37.0\%} \\
&ViLT  &76.13 &64.85 &69.66 &66.76 &65.64 &65.56 &\textbf{65.14} &68.96 &73.36 &71.35 &72.53 &75.14 &75.86 &74.27 &72.58 &\underline{77.00} &75.70 &70.90 &\textcolor{blue}{$\downarrow$ 6.9\%} \\
&TCL  &81.33 &\textbf{71.16} &76.31 &72.35 &71.56 &71.90 &72.07 &75.49 &80.03 &78.80 &78.78 &\underline{82.88} &82.46 &81.52 &80.25 &82.28 &81.53 &72.37 &\textcolor{blue}{$\downarrow$ 11.0\%} \\
&BLIP  &83.08  &\textbf{67.69} &85.64 &67.18 &67.69 &75.90 & 74.87 &69.23 &72.82 &78.46 &83.59 &83.59 & 79.49 &\underline{87.18} &82.05 &82.05 &74.36  &76.99   &\textcolor{blue}{$\downarrow$ 7.3\%}       \\ 
&METER &83.05 &73.10 &77.63 &74.05 &72.49 &\textbf{70.64} &74.27 &76.10 &79.62 &75.96 &78.55 &\underline{82.58} &81.87 &80.42 &79.52 &82.34 &81.45 &77.54 &\textcolor{blue}{$\downarrow$ 6.6\%} \\
\midrule
\multirow{3}{*}{SNLI-VE-test} 
&ALBEF &80.91 &\textbf{64.87} &71.90 &65.99 &65.03 &66.91 &67.27 &74.77 &74.93 &74.90 &78.44 &\underline{80.20} &\underline{80.20} &\underline{80.20} &\underline{80.20} &\underline{80.20} &77.31 &73.96 &\textcolor{blue}{$\downarrow$ 8.6\%} \\
&TCL  &80.29 &\textbf{65.27} &71.83 &65.81 &64.66 &67.69 &67.25 &74.59 &73.70 &74.49 &78.01 &79.77 &79.77 &79.77 &\underline{79.84} &\underline{79.84} &76.62 &73.67 &\textcolor{blue}{$\downarrow$ 8.2\%} \\
&METER &81.19 &\textbf{66.09} &74.26 &67.39 &66.30 &68.92 &69.71 &74.88 &73.89 &72.95 &78.38 &76.65 &80.96 &80.83 &\underline{81.21} &81.05 &77.14 &74.41 &\textcolor{blue}{$\downarrow$ 8.4\%} \\
\bottomrule
\end{tabular}

==> tables/unimodal/vision_error.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
\textbf{Model/corruption} &\textbf{bright} &\textbf{contrast} &\textbf{defocus} &\textbf{elastic} &\textbf{fog} &\textbf{glass} &\textbf{gauss} &\textbf{impulse} &\textbf{jpeg} &\textbf{motion} &\textbf{pixelate} &\textbf{saturate} &\textbf{shot} &\textbf{snow} &\textbf{spatter} &\textbf{speckle} &\textbf{zoom} \\
\midrule
deit\_base\_distilled &0.06 &0.03 &0.09 &0.11 &0.03 &0.10 &0.02 &0.02 &0.08 &0.07 &0.06 &0.06 &0.03 &0.07 &0.06 &0.04 &0.11 \\
densenet169 &0.06 &0.07 &0.11 &0.16 &0.09 &0.17 &0.16 &0.18 &0.09 &0.17 &0.12 &0.07 &0.17 &0.18 &0.15 &0.15 &0.17 \\
eca\_nfnet\_l0 &0.13 &0.30 &0.07 &0.08 &0.43 &0.08 &0.07 &0.09 &0.07 &0.07 &0.08 &0.10 &0.06 &0.13 &0.14 &0.06 &0.06 \\
efficientnetv2 &0.10 &0.22 &0.06 &0.09 &0.13 &0.07 &0.06 &0.06 &0.07 &0.07 &0.06 &0.10 &0.06 &0.06 &0.08 &0.07 &0.06 \\
gmlp\_s16\_224 &0.04 &0.20 &0.09 &0.09 &0.10 &0.09 &0.04 &0.04 &0.06 &0.06 &0.05 &0.05 &0.04 &0.14 &0.08 &0.04 &0.14 \\
mixer\_b16\_224 &0.13 &0.30 &0.18 &0.24 &0.09 &0.17 &0.21 &0.23 &0.23 &0.22 &0.18 &0.17 &0.21 &0.27 &0.22 &0.22 &0.31 \\
mobilenetv3\_large &0.07 &0.06 &0.05 &0.06 &0.05 &0.07 &0.04 &0.04 &0.04 &0.04 &0.04 &0.06 &0.04 &0.06 &0.05 &0.03 &0.04 \\
pit\_s\_224 &0.09 &0.40 &0.06 &0.08 &0.49 &0.07 &0.19 &0.19 &0.04 &0.05 &0.05 &0.07 &0.14 &0.06 &0.09 &0.11 &0.05 \\
regnety\_064 &0.06 &0.09 &0.08 &0.13 &0.09 &0.10 &0.15 &0.17 &0.09 &0.14 &0.13 &0.07 &0.16 &0.17 &0.11 &0.15 &0.14 \\
resmlp\_24\_224 &0.09 &0.36 &0.06 &0.07 &0.38 &0.07 &0.16 &0.16 &0.04 &0.05 &0.07 &0.07 &0.14 &0.05 &0.08 &0.14 &0.04 \\
resnet50d &0.10 &0.29 &0.07 &0.10 &0.30 &0.08 &0.07 &0.08 &0.06 &0.06 &0.07 &0.09 &0.07 &0.06 &0.12 &0.06 &0.05 \\
resnext101\_32x8d &0.10 &0.16 &0.12 &0.18 &0.14 &0.16 &0.24 &0.25 &0.13 &0.16 &0.15 &0.11 &0.25 &0.24 &0.17 &0.20 &0.17 \\
swin\_small\_patch4 &0.06 &0.24 &0.06 &0.08 &0.46 &0.08 &0.26 &0.21 &0.05 &0.05 &0.06 &0.04 &0.18 &0.04 &0.12 &0.16 &0.06 \\
vit\_small\_patch16 &0.05 &0.05 &0.06 &0.09 &0.03 &0.06 &0.08 &0.09 &0.05 &0.06 &0.05 &0.07 &0.07 &0.15 &0.08 &0.08 &0.13 \\
\bottomrule
\end{tabular}

==> tables/unimodal/vision_likelihood.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrr}
\toprule
\textbf{Model/corruption} &\textbf{bright} &\textbf{contrast} &\textbf{defocus} &\textbf{elastic} &\textbf{fog} &\textbf{galass} &\textbf{gauss} &\textbf{impulse} &\textbf{jpeg} &\textbf{motion} &\textbf{pixelate} &\textbf{saturate} &\textbf{shot} &\textbf{snow} &\textbf{spatter} &\textbf{speckle} &\textbf{zoom} \\
\midrule
deit\_base\_distilled &0.75 &0.75 &2.06 &1.83 &0.87 &2.05 &1.47 &1.51 &1.34 &1.67 &1.52 &0.80 &1.54 &1.46 &1.12 &1.21 &2.29 \\
densenet169 &1.18 &1.81 &3.01 &3.17 &1.86 &3.47 &3.19 &3.51 &2.02 &3.55 &2.40 &1.33 &3.32 &3.24 &2.59 &2.80 &3.39 \\
eca\_nfnet\_l0 &0.95 &1.48 &2.71 &2.55 &2.18 &2.64 &3.59 &3.25 &1.63 &1.97 &2.73 &0.97 &3.61 &1.90 &1.35 &2.28 &2.42 \\
efficientnetv2 &1.01 &1.73 &2.53 &2.42 &2.13 &2.48 &3.18 &2.90 &1.54 &2.03 &2.05 &1.07 &3.09 &1.93 &1.37 &2.02 &2.40 \\
gmlp\_s16\_224 &1.26 &1.65 &3.06 &2.20 &1.77 &2.86 &2.19 &2.29 &1.90 &2.41 &2.01 &1.33 &2.28 &3.71 &1.92 &1.81 &3.39 \\
mixer\_b16\_224 &1.45 &1.98 &4.03 &3.42 &2.07 &3.80 &4.60 &5.06 &3.19 &3.42 &2.89 &1.93 &4.83 &4.05 &2.87 &3.76 &4.73 \\
mobilenetv3\_large &1.23 &2.91 &3.42 &2.80 &2.35 &3.32 &3.90 &3.71 &1.98 &2.64 &2.78 &1.41 &3.86 &3.30 &2.18 &2.74 &3.15 \\
pit\_s\_224 &0.98 &1.66 &2.59 &2.36 &2.18 &2.56 &1.94 &2.01 &1.49 &2.08 &2.12 &1.02 &1.92 &1.82 &1.43 &1.54 &2.85 \\
regnety\_064 &1.03 &2.27 &2.75 &2.69 &1.79 &2.84 &3.23 &3.34 &1.92 &2.98 &2.99 &1.25 &3.49 &2.98 &1.87 &2.82 &2.93 \\
resmlp\_24\_224 &1.09 &1.81 &2.71 &2.29 &2.51 &2.58 &2.36 &2.47 &1.88 &2.18 &2.33 &1.14 &2.44 &2.20 &1.75 &1.94 &2.78 \\
resnet50d &1.01 &1.46 &2.91 &3.07 &1.79 &2.81 &3.46 &3.52 &1.69 &2.65 &3.32 &1.08 &3.39 &2.56 &1.85 &2.41 &2.80 \\
resnext101\_32x8d &1.19 &2.63 &2.66 &2.74 &2.01 &3.00 &3.79 &4.12 &1.89 &2.64 &2.28 &1.45 &4.01 &3.61 &2.38 &2.92 &2.77 \\
swin\_small\_patch4 &0.85 &1.16 &2.45 &2.33 &1.91 &2.57 &2.22 &2.17 &2.09 &1.93 &3.51 &0.89 &2.12 &1.62 &1.10 &1.59 &2.41 \\
vit\_small\_patch16 &1.70 &1.15 &2.77 &2.53 &1.36 &2.63 &3.76 &4.00 &2.01 &2.27 &1.87 &2.09 &4.02 &4.53 &2.23 &2.99 &3.37 \\
\bottomrule
\end{tabular}
